ByteFS: System Support for (CXL-based) Memory-Semantic Solid-State Drives

Unlike non-volatile memory that resides on the processor memory bus, memory-semantic solid-state drives (SSDs) support both byte and block access granularity via PCIe or CXL interconnects. They provide scalable memory capacity using NAND flash at a much lower cost. In addition, they have different performance characteristics for their dual byte/block interface respectively, while offering essential memory semantics for upper-level software. Such a byte-accessible storage device provides new implications on the software system design. In this paper, we develop a new file system, named ByteFS, by rethinking the design primitives of file systems and SSD firmware to exploit the advantages of both byte and block-granular data accesses. ByteFS supports byte-granular data persistence to retain the persistence nature of SSDs. It extends the core data structure of file systems by enabling dual byte/block-granular data accesses. To facilitate the support for byte-granular writes, \pname{} manages the internal DRAM of SSD firmware in a log-structured manner and enables data coalescing to reduce the unnecessary I/O traffic to flash chips. ByteFS also enables coordinated data caching between the host page cache and SSD cache for best utilizing the precious memory resource. We implement ByteFS on both a real programmable SSD and an emulated memory-semantic SSD for sensitivity study. Compared to state-of-the-art file systems for non-volatile memory and conventional SSDs, ByteFS outperforms them by up to 2.7$\times$, while preserving the essential properties of a file system. ByteFS also reduces the write traffic to SSDs by up to 5.1$\times$ by alleviating unnecessary writes caused by both metadata and data updates in file systems.

==> discuss.tex <==
\section{Discussion}
\label{sec:discuss}

%\jian{Wear leveling and privacy should be in the Design section. We will discuss how our proposed techniques will not hurt existing wear leveling schemes. How we 
%erase the flash blocks to ensure the data privacy.  }

\noindent
\textbf{Implication for Applications.}
\vspace{20ex}
Discuss the implications we have on applications that can design around harvesting storage


%\noindent
%\textbf{ML Accuracy vs. Harvesting Efficiency.}
%\vspace{20ex}
%
%\subsection{Wear Leveling}
%\vspace{20ex}
%Discuss wear leveling concerns
%
%\subsection{Privacy}
%\vspace{20ex}
%Discuss possible data privacy concerns about giving away storage


==> revisionplan.tex <==
\onecolumn
\thispagestyle{plain}
% \pagestyle{plain}

% \pagenumbering{arabic}

% \setstretch{0.9}

\centerline{\LARGE \textbf{Revision Log for \pname}}
\vspace{1ex}
\noindent {\large {\hlcommon{\textbf{Common Concerns}}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Novelty of ByteFS}

We elaborated on the design challenges of ByteFS and the technical contributions we made in sections \S\ref{sec:intro} and \S\ref{sec:design}.

\item \textbf{Evaluation Baselines}

We clarified the baseline filesystem selection in \S\ref{subsec:eva_setup}.

\item \textbf{M-SSD Setting}

We clarified the M-SSD setting used in baseline file systems and ByteFs in the evaluation section \S\ref{subsec:eva_setup}. We will clarify the cache scheme and detailed memory usage.

\item \textbf{CoW Memory Usage}

We added the CoW memory usage numbers in \S\ref{subsec:dataio} to show its low overhead.

\end{enumerate}

% ----- reviewer A ------

\noindent {\large {\hlA{\textbf{Reviewer A}}}}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{M-SSD Use Case}

We clarified the M-SSD can be used as a memory expander via memory mapping of ByteFS in \S\ref{subsec:dataio}.

\item \textbf{Traffic Breakdown Setting in Figure~\ref{fig:motivation_breakdown}}

We clarified the setting of the traffic breakdown in the caption of Figure~\ref{fig:motivation_breakdown} and \S\ref{sec:study}. 

\item \textbf{Range Lookup Complexity}

We clarified how SSD firmware performs a single range lookup that overlaps partitions in \S\ref{subsec:log}.

\item \textbf{Memory Footprint of the Log Index}

We clarified the factors that affect the log index space cost in \S\ref{subsec:log}.

\end{enumerate}

% ----- reviewer B ------

\noindent {\large {\hlB{\textbf{Reviewer B}}}}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{M-SSD Hardware Assumptions}

We clarified the hardware assumption of mSSD in \S\ref{subsec:bytessd}.

\item \textbf{Clarification on Coordinate Caching}

We clarified the coordinate caching in \S\ref{subsec:log}. 

\item \textbf{Study Section}

We elaborated on how the profiled study guides us to examine the design tradeoffs of using byte/block interface in \S\ref{sec:study}.

\item \textbf{Necessity of clflush/clwb}

We clarified the reason for using clflush/clwb as a persistence barrier to ensure the buffered data is flushed to M-SSD in \S\ref{subsec:enable_interface}.

\item \textbf{Difference between Ext4 vs. ByteFS}

We clarified the key changes we made from Ext4 in \S\ref{subsec:impl}.

\end{enumerate}

% ----- reviewer C ------

\noindent {\large {\hlC{\textbf{Reviewer C}}}}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

% \item \textbf{Difference between Ext4 vs. ByteFS}

\item \textbf{Log Space Management}

We clarified the log cleaning in ByteFS and how ByteFS splits the operation into smaller atomic operations at block granularity in \S\ref{subsec:log}.

\item \textbf{Flushing Dirty Pages from Host Memory}

We clarified the page writeback trigger policy and transaction procedure in ByteFS in \S\ref{subsec:dataio}. 

\item \textbf{Ext4 with Journal Placed In the SSD DRAM}

We clarified the baseline cache setting in \S\ref{subsec:eva_setup}.

\item \textbf{File System Size And Workload Size}

We clarified the baseline and ByteFS file system size in \S\ref{subsec:eva_setup}.

\item \textbf{Value Size in YCSB}

We clarified the default size of key/value records in YCSB benchmarks in Table~\ref{tab:workloads}. 

\item \textbf{Differences in Metadata Read Traffic Between Ext4 and ByteFS}

We extended the discussion on why ByteFS significantly reduces the metadata read traffic as shown in Figure~\ref{fig:external_traffic_micro} in \S\ref{subsec:external_traffic}.

\item \textbf{Clarification on Figure~\ref{fig:perf_break}}

We clarified the differences and techniques deployed in ByteFS-Dual, ByteFS-Log, and ByteFS when evaluating the performance breakdown of ByteFS in \S\ref{subsec:perf_break}.

\item \textbf{Paper Title}

We made the title more informative.

\item \textbf{In-Device Memory for FTL}

We clarified how the SSD DRAM is consumed in our M-SSD setting in \S\ref{subsec:impl}.

\item \textbf{I/O Amplification}

We clarified how I/O amplification is measured and calculated in \S\ref{subsec:io_amplification}.

\item \textbf{Same Page/Block Written by Two Transactions}

We clarified how ByteFS tracks different versions of updates within the same page in the log region in \S\ref{subsec:dual_support}.

\item \textbf{Commit Ordering During Flushing}

We clarified how ByteFS flushes committed data in commit order as logged in TxLog in \S\ref{subsec:log}.

\item \textbf{Write Buffer in SSD}

We clarified the SSD write buffer functionality in \S\ref{subsec:log}. 

\item \textbf{Integrating JBD2}

We clarified how we reuse the transaction management mechanism in JBD2 in section \S\ref{subsec:dataio}.

 \item \textbf{Interface Selection}
 
We discussed the byte/block cutoff and clarify the interface selection for different data structures in \S\ref{sec:study}.

\item \textbf{Double Logging}

We clarified the “double logging” term in \S\ref{subsec:log}.


\end{enumerate}

% ----- reviewer D ------

\noindent {\large {\hlD{\textbf{Reviewer D}}}}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Baseline M-SSD}

We extended the discussion on the limitation of the baseline M-SSD design in \S\ref{subsec:bytessd}.

\item \textbf{Performance Breakdown}

We clarified the differences and techniques deployed in ByteFS-Dual, ByteFS-Log, and ByteFS when evaluating the performance breakdown of ByteFS in \S\ref{subsec:perf_break}.

\item \textbf{Clarification on Read Latency}

We clarified the read latency in \S\ref{subsec:bytessd}. We clarified the reported latency in Figure~\ref{fig:ycsb_latency} as average end-to-end latency in \S\ref{subsec:overall_perf}. 

\item \textbf{Related Work}

We discussed the relevant studies of tiered memory in our related work in \S\ref{sec:related}.


\end{enumerate}

% ----- reviewer E ------

\noindent {\large {\hlE{\textbf{Reviewer E}}}}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Profiling Study in Section~\ref{sec:study}}

We elaborated the motivation of the study in \S\ref{sec:study}.

\item \textbf{I/O Interface Choices}

We extended the discussion of the performance benefits of exploiting the data locality of the metadata cache in the host in \S\ref{sec:study}.

\item \textbf{Clarification on the Assumptions of M-SSDs}

We clarified the firmware changes in ByteFS does not require hardware changes and can be easily deployed by SSD vendors in \S\ref{subsec:impl}.

\item \textbf{M-SSD Implementation}

We elaborated the essential techniques we used to build the M-SSD prototype in \S\ref{subsec:enable_interface}.

\item \textbf{Challenges and Considerations for In-Device Log}

We clarified the goals and challenges of designing the firmware-level logging, and discussed the core designs we made to achieve them in \S\ref{subsec:log}.

\item \textbf{Coherence with Cacheable MMIO Region}

We clarified that there is no coherence issue between the host CPU and M-SSD with cacheable MMIO region since M-SSD firmware does not modify the data read/written by the host in \S\ref{subsec:enable_interface}.

\item \textbf{Three-Layer Indexing Structure}

We extended the discussion of why we split the indexing structure into multiple layers in \S\ref{subsec:log}. 

\item \textbf{Importance of Arbitrary Chunk Sizes and Range Lookup}

We extended the discussion of why we need to support arbitrary chunk sizes in the log region and support range lookup in \S\ref{subsec:log}. 

 \item \textbf{ARM Processor Used in M-SSD}
 
We added the background information of the FPGA board used in our SSD prototype in \S\ref{subsec:impl}.

 \item \textbf{Power Failure} 
 
We clarified the recovery procedure after Power Failure in \S\ref{subsec:consistency}.

\item \textbf{Log Cleaning}

We clarified the Log-cleaning procedure and how transactions are correctly handled in \S\ref{subsec:log}.

\item \textbf{Atomic and Concurrent Read/Write}

We clarified how ByteFS relies on the filesystem transaction to ensure the atomicity of concurrent reads/writes in \S\ref{subsec:dual_support}.

\item \textbf{Inode Updates}

We clarified why ByteFS is still able to coalesce inode changes with the log region in \S\ref{subsec:log} and \S\ref{subsec:put_together}.

\item \textbf{NOVA and PMFS for M-SSD}

We clarified how we set up the NOVA and PMFS to use M-SSD in \S\ref{subsec:eva_setup}.

\item \textbf{Parallel Accesses on M-SSD}

We clarified that M-SSD supports concurrent access via the PCIe MMIO interface in \S\ref{subsec:enable_interface}.

\item \textbf{Clarification on the I/O Traffic in PMFS}

We clarified the detailed reason why PMFS incurs higher I/O traffic than ByteFS in \S\ref{subsec:perf_break}.

\item \textbf{Host-Side Metadata Caching}

We clarified the term “Host-Side Metadata Caching” in \S\ref{subsec:selection}.

\item \textbf{Dual Interface Implementation in Other File Systems}

We clarified it is hard to leverage byte/block interface in existing filesystems without changing the inherent design in \S\ref{subsec:why}. We also clarified the interface set up of the other file system in \S\ref{subsec:eva_setup}.

\item \textbf{Comparing ByteFS with FlatFlash}

We extended the discussion of FlatFlash in the related work in \S\ref{sec:related}.

\item \textbf{Responsibilities of the Hardware and the Software}

We clarified for each proposed technique whether it is in firmware or the host file system in \S\ref{sec:design}.


\end{enumerate}
